Symmetry in Multiple Self-Consistent-Field Solutions of Transition-Metal Complexes

We use a method based on metadynamics to locate multiple low-energy Unrestricted Hartree--Fock (UHF) self-consistent-field (SCF) solutions of two model octahedral $d^1$ and $d^2$ transition-metal complexes, $[\mathrm{MF}_6]^{3-} (\mathrm{M} = \mathrm{Ti}, \mathrm{V})$. By giving a group-theoretical definition of symmetry breaking, we classify these solutions in the framework of representation theory and observe that a number of them break spin or spatial symmetry, if not both. These solutions seem unphysical at first, but we show that they can be used as bases for Non-Orthogonal Configuration Interaction (NOCI) to yield multi-determinantal wavefunctions that have the right symmetry to be assigned to electronic terms. Furthermore, by examining the natural orbitals and occupation numbers of these NOCI wavefunctions, we gain insight into the amount of static correlation that they incorporate. We then investigate the behaviors of the most low-lying UHF and NOCI wavefunctions when the octahedral symmetry of the complexes is lowered and deduce that the symmetry-broken UHF solutions must first have their symmetry restored by NOCI before they can describe any vibronic stabilization effects dictated by the Jahn--Teller theorem.

==> Makefile <==
LATEXMK=latexmk
MAIN=symmultiplescf-arxiv
TEXSOURCES:=$(MAIN).tex $(wildcard */*.tex)
TIKZSOURCES:=$(shell find -name "*.tikz")
PLOTSOURCES:=$(shell find -name "*.csv")
IMAGESOURCES:=$(shell find -name "*.eps")
SOURCES=$(TEXSOURCES) $(TIKZSOURCES) $(PLOTSOURCES) $(IMAGESOURCES) Makefile


all: $(SOURCES) notikzex

cleanaux:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.auxlock *.end *.fls *.log *.out *.fdb_latexmk *.synctex.gz

cleanall: cleanaux

tikzex:
	$(LATEXMK) -quiet -lualatex \
			-pdflualatex="lualatex --shell-escape --synctex=1 --interaction=nonstopmode %O %S" $(MAIN).tex

notikzex:
	$(LATEXMK) -quiet -pdf \
			-pdflatex="pdflatex --shell-escape --synctex=1 --interaction=nonstopmode %O '\def\notikzex{1}\input{%S}'" $(MAIN).tex

.PHONY: all cleanaux cleanall tikzex notikzex


==> apps/apps.tex <==









==> introduction/tikz/AAdashtetoct.tex <==
\begin{tikzpicture}[%
	rotate around y=-15,%
	scale = 1.0,%
	every node/.style={scale=0.56},%
	]
	% A
	%% Coord def
	\coordinate (A1) at (0,-0.83,2);
	\coordinate (A2) at (0,-0.83,-2);
	\coordinate (A3) at (2, 2, 0);
	\coordinate (A4) at (-2, 2, 0);
	% Adash
	%% Coord def
	\coordinate (Adash1) at ($(A2)!0.5!(A4)$);
	\coordinate (Adash2) at ($(A2)!0.5!(A3)$);
	\coordinate (Adash3) at ($(A1)!0.5!(A2)$);
	\coordinate (Adash4) at ($(A1)!0.5!(A3)$);
	\coordinate (Adash5) at ($(A1)!0.5!(A4)$);
	\coordinate (Adash6) at ($(A3)!0.5!(A4)$);
	%% Orbitals
	\draw[->, shorten >=0.15cm, densely dotted] ($(A1) + (0,1,2.1)$) -- (A1);
	\draw[->, shorten >=0.15cm, densely dotted] ($(Adash1) + (1,1.6,0)$) .. controls ($(Adash2)!0.5!(Adash6)$) and ($(Adash2)!0.5!(Adash6)$) .. (Adash1);
	\node[draw, densely dotted, anchor = south] (AdashEorb) at ($(A1) + (0,1,2.1)$) {\includegraphics[width=.08\textwidth, trim=0 0 0 -5]{plots/A_o161_39.png} \quad \includegraphics[width=.08\textwidth]{plots/A_o161_40.png}};
	\node[draw, densely dotted, anchor = south] (AdashEorb) at ($(Adash1) + (1,1.6,0)$) {\includegraphics[width=.08\textwidth, trim=0 0 0 -5]{plots/Adash_o42_39.png} \quad \includegraphics[width=.08\textwidth]{plots/Adash_o42_40.png}};
	%% Draw lines
	\draw[blue, thick] (A1) -- (A2);
	\draw[blue, thick] (A1) -- (A4);
	\draw[blue, thick] (A2) -- (A3);
	\draw[blue, thick] (A3) -- (A4);
	\draw[blue, thick, densely dashed] (A2) -- (A4);
	\draw[red, thin] (Adash5) -- (Adash4);
	\draw[red, thin] (Adash5) -- (Adash6);
	\draw[red, thin, densely dashed] (Adash5) -- (Adash1);
	\draw[red, thin, densely dashed] (Adash5) -- (Adash3);
	\draw[red, thin] (Adash6) -- (Adash4);
	\draw[red, thin, densely dashed] (Adash6) -- (Adash2);
	\draw[red, thin, densely dashed] (Adash6) -- (Adash1);
	\draw[red, thin, densely dashed] (Adash6) -- (Adash1);
	\draw[red, thin] (Adash4) -- (Adash3);
	\draw[red, thin] (Adash4) -- (Adash2);
	\draw[red, thin] (Adash3) -- (Adash2);
	\draw[red, thin, densely dashed] (Adash3) -- (Adash1);
	\draw[red, thin, densely dashed] (Adash2) -- (Adash1);
	\draw[blue, thick] (A1) -- (A3);
	%% Plot states
	\foreach \astate in {A1, A2, A3, A4} \draw [fill=blue, draw=black] (\astate) circle [radius=.05];
	\foreach \adashstate in {Adash1, Adash2, Adash3, Adash4, Adash5, Adash6} \draw [fill=red, draw=black] (\adashstate) circle [radius=.05];
	%% Label states
	\node[anchor = north east, blue] (AElabel) at (A1) {$\mathrm{A}_1$};
	\node[anchor = north west, blue] (AC21label) at (A2) {$\mathrm{A}_2$};
	\node[anchor = south west, blue] (AC24label) at (A3) {$\mathrm{A}_3$};
	\node[anchor = south east, blue] (AC21label) at (A4) {$\mathrm{A}_4$};
	\node[anchor = north east, red] (AdashElabel) at ($(Adash1)+(0.11,0,0)$) {$\mathrm{A}'_1$};
	\node[anchor = west, inner sep = 4pt, red] (AdashC30label) at (Adash2) {$\mathrm{A}'_2$};
	\node[anchor = north, inner sep = 6pt, red] (AdashCm30label) at (Adash3) {$\mathrm{A}'_3$};
	\node[anchor = north west, red, inner sep = 1pt] (AdashC41label) at (Adash4) {$\mathrm{A}'_4$};
	\node[anchor = east, inner sep = 4pt, red] (AdashC4130label) at (Adash5) {$\mathrm{A}'_5$};
	\node[anchor = south, red] (AdashC41m30label) at (Adash6) {$\mathrm{A}'_6$};
\end{tikzpicture}

==> suppinfo/Makefile <==
LATEXMK=latexmk
MAIN=symmultiplescf-suppinfo
TEXSOURCES:=$(MAIN).tex qchemlanguage.tex $(wildcard */*.tex)
SNIPPETSOURCE:=$(shell find -name "*.inp")
TIKZSOURCES:=$(shell find -name "*.tikz")
PLOTSOURCES:=$(shell find -name "*.csv")
IMAGESOURCES:=$(shell find -name "*.eps")
SOURCES=$(TEXSOURCES) $(SNIPPETSOURCES) $(TIKZSOURCES) $(PLOTSOURCES) $(IMAGESOURCES) Makefile


all: $(SOURCES) lualatex

cleanaux:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.auxlock *.end *.fls *.log *.out *.fdb_latexmk *.synctex.gz

cleanall: cleanaux

lualatex:
	$(LATEXMK) -quiet -lualatex \
			-pdflualatex="lualatex --shell-escape --synctex=1 --interaction=nonstopmode %O %S" $(MAIN).tex

pdflatex:
	$(LATEXMK) -quiet -pdf \
			-pdflatex="pdflatex --shell-escape --synctex=1 --interaction=nonstopmode %O %S" $(MAIN).tex

.PHONY: all cleanaux cleanall lualatex pdflatex


==> suppinfo/qchemlanguage.tex <==
% !TeX root = symmultiplescf-suppinfo.tex

\definecolor{eclipseBlue}{RGB}{42,0.0,255}
\definecolor{eclipseGreen}{RGB}{63,127,95}
\definecolor{eclipsePurple}{RGB}{127,0,85}

\lstdefinelanguage{QChemInput}
{
	%% List of keywords
	alsoletter = {_\$},
	% Rem variables
	keywords = [1]{
		SCF_MINFIND_INITNORM,
		BASIS,
		EXCHANGE,
		CORRELATION,
		UNRESTRICTED,
		SCF_GUESS,
		SCF_CONVERGENCE,
		SCF_ALGORITHM,
		SCF_MAX_CYCLES,
		MOM_START,
		PRINT_ORBITALS,
		SCF_PRINT,
		MAX_SCF_CYCLES,
		SYMMETRY,
		THRESH,
		DIIS_SEPARATE_ERRVEC,
		SYM_IGNORE,
		SCF_SAVEMINIMA,
		SCF_READMINIMA,
		SCF_MINFIND_INITNORM,
		SCF_MINFIND_INCREASEFACTOR,
		SCF_MINFIND_WELLTHRESH,
		SCF_MINFIND_RANDOMMIXING,
		SCF_MINFIND_NRANDOMMIXES,
		SCF_MINFIND_MIXMETHOD,
		SCF_MINFIND_MIXENERGY,
		SCF_MINFIND_RESTARTSTEPS,		
	},
	keywords = [2]{
		\$molecule,
		\$rem,
		\$rem_frgm,
		\$occupied,
		\$end,
	},
	comment = [l]{!},
	% Style
	sensitive = false, % keywords are not case-sensitive
	caption = \lstname,
	backgroundcolor = \color{Cornsilk},
	frame = trbl,
	numberstyle = \tiny\ttfamily\noncopy, % style of the line numbers
	numbers = left,
	% Syntax highlighting
	keywordstyle = [1]{\color{eclipsePurple}},
	keywordstyle = [2]{\color{Navy}},
	commentstyle = \color{eclipseGreen}
}

\newcommand*{\qchemsection}[1]{{\color{Navy} \texttt{\$#1}}}
\newcommand*{\qchemremvar}[1]{{\color{eclipsePurple} \texttt{#1}}}

\lstdefinestyle{custombash}{
	language = bash,
	frame = trbl,
	backgroundcolor = \color{Seashell},
%	breakatwhitespace = true,
	breaklines = true,
	prebreak = \mbox{\textcolor{red}{\textbackslash}},
	postbreak = \mbox{\textcolor{Green}{\noncopy{>}}},
}

\lstdefinelanguage{QChemOutput}
{
	%% List of keywords
	alsoletter = {},
	keywords = [1]{
	},
	% Style
	sensitive = false, % keywords are not case-sensitive
	caption = \lstname,
	backgroundcolor = \color{Cornsilk},
	frame = trbl,
	numberstyle = \tiny\ttfamily\noncopy, % style of the line numbers
	numbers = left,
	% Syntax highlighting
}
